Robust Algorithms for TSP and Steiner Tree

Robust optimization is a widely studied area in operations research, where the algorithm takes as input a range of values and outputs a single solution that performs well for the entire range. Specifically, a robust algorithm aims to minimize regret, defined as the maximum difference between the solution's cost and that of an optimal solution in hindsight once the input has been realized. For graph problems in P, such as shortest path and minimum spanning tree, robust polynomial-time algorithms that obtain a constant approximation on regret are known. In this paper, we study robust algorithms for minimizing regret in NP-hard graph optimization problems, and give constant approximations on regret for the classical traveling salesman and Steiner tree problems.

==> steiner.tex <==
\section{Algorithm for the Robust Steiner Tree Problem}\label{section:steiner}

\begin{figure}
\begin{center}
 \textbf{Minimize } $r$ \textbf{subject to}
\begin{eqnarray} 
\label{eq:steiner}\forall S \subset V \text{ such that } \emptyset \subset S \cap T \subset T: &\sum_{e \in \delta(S)} x_e \geq 1\\
\label{eq:range}\forall \bd \text{ such that } d_e \in [\ell_e, u_e]: & \sum_{e \in E} d_e x_e \leq \opt(\bd) + r\\
\forall e \in E: & x_e \in [0, 1] 
\end{eqnarray}
\end{center}
\caption{The Robust Steiner Tree Polytope}
\label{fig:rrst}
\end{figure}

In this section, our goal is to find a fractional solution to the LP in Fig.~\ref{fig:rrst} for robust Steiner tree. By Theorem~\ref{thm:generalrounding} and known approximation/integrality gap results for Steiner Tree, this gives the following theorem:

\begin{theorem}\label{thm:steiner-main}
There exists a $(2755, 64)$-robust algorithm for the Steiner tree problem.
\end{theorem}

It is well-known that the standard Steiner tree polytope admits an exact separation oracle
(by solving the $s, t$-min-cut problem using edge weights $x_e$ for all $s, t \in T$) so it is sufficient to find an approximate separation oracle for the regret constraint set. We present the main ideas of the separation oracle here, and defer the details to Appendix~\ref{section:deferred-st}.

First, we create the derived instance of the Steiner tree problem which is a copy $G'$ of the input graph $G$ with edge weights $u_e x_e +\ell_e -\ell_e x_e$. As noted earlier, the optimal Steiner tree $T^*$ on the derived instance maximizes the regret of the fractional solution $\bx$. However, since Steiner tree is \np-hard, we cannot hope to exactly find $T^*$. We need a Steiner tree $\hat{T}$ such that the regret caused by it can be bounded against that caused by $T^*$. The difficulty is that the regret corresponds to the total weight of edges \textit{not} in the Steiner tree (plus an offset that we will address later), whereas standard Steiner tree approximations give guarantees in terms of the total weight of edges in the Steiner tree. 
%So, a standard approximation algorithm that bounds the weight of edges in $T$ against that in $T^*$ does not suffice.
%
We overcome this difficulty by requiring a stricter notion of ``difference approximation'' -- that the weight of edges $\hat{T} \setminus T^*$ be bounded against those in $T^* \setminus \hat{T}$. Note that this condition ensures that not only is the weight of edges in $\hat{T}$ bounded against those in $T^*$, but also that the weight of edges {\em not in $\hat{T}$} is bounded against that of edges {\em not in $T^*$}. We show the following lemma to obtain the difference approximation:

\begin{lemma}\label{lemma:differenceapprox}
For any $\epsilon > 0$, there exists a polynomial-time algorithm for the Steiner tree problem such that if $\opt$ denotes the set of edges in the optimal solution and $c(S)$ denotes the total weight of edges in $S$, then for any input instance of Steiner tree, the output solution $\alg$ satisfies $c(\alg \setminus \opt) \leq (4 + \epsilon) \cdot c(\opt \setminus \alg)$.
\end{lemma}

The algorithm proving Lemma~\ref{lemma:differenceapprox} is a local search procedure proposed by \cite{GGKMSSV17} that considers local moves of the following form: For the current solution $\alg$, a local move consists of adding any path $f$ whose endpoints are vertices in $\alg$ and whose intermediate vertices are not in $\alg$, and then deleting from $\alg$ a subpath $a$ in the resulting cycle such that $\alg \cup f \setminus a$ remains feasible. We extend the results in \cite{GGKMSSV17} by showing in Section~\ref{section:localsearch} that such an algorithm is 4-approximate.
%The high-level idea of their proof is to show that for $\alg$ and any $\sol$, there is a decomposition of $\alg$ into paths $S$ and a fractional charging from these paths to paths $f$ in $\sol$ such that (a) any $S$ is only fractionally charged to $f$ such that $S$ and $f$ can be swapped in a local move and (b) the sum over all $S$ of the fraction of $S$ charged to $f$ is at most 14. The approximation ratio immediately follows by using the local optimality of $\alg$. 
We can further extend this argument to show that such an algorithm, in fact, satisfies the stricter difference approximation requirement in Lemma~\ref{lemma:differenceapprox} (see Section~\ref{section:deferred-st} for details).

Recall that the regret caused by $T$ is not exactly the weight of edges not in $T$, but includes a fixed offset of $\sum_{e \in E} (\ell_e - \ell_e x_e)$. If $\ell_e = 0$ for all edges, i.e., the offset is $0$, then we can recover a robust algorithm from Lemma~\ref{lemma:differenceapprox} alone with much better constants than in Theorem~\ref{thm:steiner-main} (we defer the discussion/proof of this result to Appendix~\ref{section:steiner-zlb}). In general though, the approximation guarantee given in Lemma~\ref{lemma:differenceapprox} alone does not suffice because of the offset. We instead rely on a stronger notion of approximation formalized in the next lemma that provides simultaneous approximation guarantees on two sets of edge weights: $c_e = u_e x_e  - \ell_e x_e + \ell_e$ and $c_e' = \ell_e - \ell_e x_e$. The guarantee on $\ell_e - \ell_e x_e$ can then be used to handle the offset.

\begin{lemma}\label{lemma:differenceapprox2}
Let $G$ be a graph with terminals $T$ and two sets of edge weights $c$ and $c'$. Let $\sol$ be any Steiner tree connecting $T$. Let $\Gamma' > 1$, $\kappa > 0$, and $0 < \epsilon < \frac{4}{35}$ be fixed constants.
Then there exists a constant $\Gamma$ (depending on $\Gamma', \kappa, \epsilon$) and an algorithm that obtains a collection of Steiner trees $\alg$, at least one of which (let us call it $\alg_i$) satisfies:
\begin{itemize}
    \item $c(\alg_i \setminus \sol) \leq 4\Gamma \cdot c(\sol \setminus \alg_i),$ and
    \item $c'(\alg_i) \leq (4\Gamma' +\kappa + 1 + \epsilon) \cdot c'(\sol)$.
\end{itemize}
\end{lemma}

The fact that Lemma~\ref{lemma:differenceapprox2} generates multiple solutions (but only polynomially many) is fine because as long as we can show that one of these solutions causes sufficient regret, our separation oracle can just iterate over all solutions until it finds one that causes sufficient regret. 

We give a high level sketch of the proof of Lemma~\ref{lemma:differenceapprox2} here, and defer the full details to Appendix~\ref{section:deferred-st}. The algorithm uses the idea of \textit{alternate minimization}, alternating between a ``forward phase'' and a ``backward phase''. The goal of each forward phase/backward phase pair is to keep $c'(\alg)$ approximately fixed while obtaining a net decrease in $c(\alg)$. In the forward phase, the algorithm greedily uses local search, choosing swaps that decrease $c$ and increase $c'$ at the best ``rate of exchange'' between the two costs (i.e., the maximum ratio of decrease in $c$ to increase in $c'$), until $c'(\alg)$ has increased past some upper threshold. Then, in the backward phase, the algorithm greedily chooses swaps that decrease $c'$ while increasing $c$ at the best rate of exchange, until $c'(\alg)$ reaches some lower threshold, at which point we start a new forward phase. 

We guess the value of $c'(\sol)$ (we can run many instances of this algorithm and generate different solutions based on different guesses for this purpose) and set the upper threshold for $c'(\alg)$ appropriately so that we satisfy the approximation guarantee for $c'$. For $c$ we show that as long as $\alg$ is not a $4\Gamma$-difference approximation with respect to $c$ then a forward/backward phase pair reduces $c(\alg)$ by a non-negligible amount (of course, if $\alg$ is a $4\Gamma$-difference approximation then we are done). This implies that after enough iterations, $\alg$ must be a $4\Gamma$-difference approximation as $c(\alg)$ can only decrease by a bounded amount. To show this, we claim that while $\alg$ is not a $4\Gamma$-difference approximation, for sufficiently large $\Gamma$ the following bounds on rates of exchange hold:

\begin{itemize} 
\item For each swap in the forward phase, the ratio of decrease in $c(\alg)$ to increase in $c'(\alg)$ is at least some constant $k_1$ times $\frac{c(\alg \setminus \sol)}{c'(\sol \setminus \alg)}$.

\item For each swap in the backward phase, the ratio of increase in $c(\alg)$ to decrease in $c'(\alg)$ is at most some constant $k_2$ times $\frac{c(\sol \setminus \alg)}{c'(\alg \setminus \sol)}$. 
\end{itemize} 
Before we discuss how to prove this claim, let us see why this claim implies that a forward phase/backward phase pair results in a net decrease in $c(\alg)$. If this claim holds, suppose we set the lower threshold for $c'(\alg)$ to be, say, $101 c'(\sol)$. That is, throughout the backward phase, we have $c'(\alg) > 101 c'(\sol)$. This lower threshold lets us rewrite our upper bound on the rate of exchange in the backward phase in terms of the lower bound on rate of exchange for the forward phase:

$$k_2 \frac{c(\sol \setminus \alg)}{c'(\alg \setminus \sol)} \leq k_2 \frac{c(\sol \setminus \alg)}{c'(\alg) - c'(\sol)} \leq k_2 \frac{c(\sol \setminus \alg)}{100 c'(\sol)} \leq  k_2 \frac{c(\sol \setminus \alg)}{100 c'(\sol \setminus \alg)} $$
$$\leq k_2 \frac{1}{4\Gamma} \frac{c(\alg \setminus \sol)}{100 c'(\sol \setminus \alg)} = \frac{k_2}{400\Gamma k_1} \cdot k_1\frac{c(\alg \setminus \sol)}{c'(\sol \setminus \alg)}.$$

In other words, the bound in the claim for the rate of exchange in the forward phase is larger than the bound for the backward phase by a multiplicative factor of $\Omega(1) \cdot \Gamma$. While these bounds depend on $\alg$ and thus will change with every swap, let us make the simplifying assumption that through one forward phase/backward phase pair these bounds remain constant. Then, the change in $c(\alg)$ in one phase is just the rate of exchange for that phase times the change in $c'(\alg)$, which by definition of the algorithm is roughly equal in absolute value for the forward and backward phase. So this implies that the decrease in $c(\alg)$ in the forward phase is $\Omega(1) \cdot \Gamma$ times the increase in $c(\alg)$ in the backward phase, i.e., the net change across the phases is a non-negligible decrease in $c(\alg)$ if $\Gamma$ is sufficiently large. Without the simplifying assumption, we can still show that the decrease in $c(\alg)$ in the forward phase is larger than the increase in $c(\alg)$ in the backward phase for large enough $\Gamma$ using a much more technical analysis. In particular, our analysis will show there is a net decrease as long as:
\begin{equation}\label{eq:maincond}
\min\left\{\frac{4\Gamma - 1}{8\Gamma} ,\frac{(4\Gamma - 1)(\sqrt{\Gamma}-1)(\sqrt{\Gamma}-1-\epsilon)\kappa}{16(1+\epsilon)\Gamma^2}\right\} - (e^{\zeta' (4\Gamma'+\kappa+1+\epsilon)} - 1) > 0,
\end{equation}
where 
$$\zeta' = \frac{4(1+\epsilon)\Gamma'}{(\sqrt{\Gamma'}-1)(\sqrt{\Gamma'}-1-\epsilon)(4\Gamma'-1)(4\Gamma-1)}.$$ 
Note that for any positive $\epsilon, \kappa, \Gamma'$, there exists a sufficiently large value of $\Gamma$ for \eqref{eq:maincond} to hold, since as $\Gamma \rightarrow \infty$, we have $\zeta' \rightarrow 0$, so that 
$$(e^{\zeta' (4\Gamma'+\kappa+1+\epsilon)} - 1) \rightarrow 0 \text{ and }$$
$$\min\left\{\frac{4\Gamma - 1}{8\Gamma} ,\frac{(4\Gamma - 1)(\sqrt{\Gamma}-1)(\sqrt{\Gamma}-1-\epsilon)\kappa}{16(1+\epsilon)\Gamma^2}\right\} \rightarrow \min\{1/2, \kappa/(4+4\epsilon)\}.$$ 
So, the same intuition holds: as long as we are willing to lose a large enough $\Gamma$ value, we can make the increase in $c(\alg)$ due to the backward phase negligible compared to the decrease in the forward phase, giving us a net decrease.

It remains to argue that the claimed bounds on rates of exchange hold. Let us argue the claim for $\Gamma = 4$, although the ideas easily generalize to other choices of $\Gamma$. We do this by generalizing the analysis of the local search algorithm. This analysis shows that if $\alg$ is a locally optimal solution, then 
$$c(\alg \setminus \sol) \leq 4\cdot c(\sol \setminus \alg),$$
i.e., $\alg$ is a 4-difference approximation of $\sol$. The contrapositive of this statement is that if $\alg$ is not a 4-difference approximation, then there is at least one swap that will improve it by some amount.  We modify the approach of~\cite{GGKMSSV17} by weakening the notion of locally optimal.  In particular, suppose we define a solution $\alg$ to be ``approximately'' locally optimal if at least half of the (weighted) swaps between paths $a$ in $\alg \setminus \sol$ and paths $f$ in $\sol \setminus \alg$ satisfy $c(a) \leq 2c(f)$ (as opposed to $c(a) \leq c(f)$ in a locally optimal solution; the choice of 2 for both constants here implies $\Gamma = 4$). Then a modification of the analysis of the local search algorithm, losing an additional factor of 4, shows that if $\alg$ is approximately locally optimal, then 
$$c(\alg \setminus \sol) \leq 16 \cdot c(\sol \setminus \alg).$$   The contrapositive of this statement, however, has a stronger consequence than before: if $\alg$ is not a 16-difference approximation, then a weighted half of the swaps satisfy $c(a) > 2c(f)$, i.e. reduce $c(\alg)$ by at least 
$$c(a) - c(f) > c(a) - c(a)/2 = c(a)/2.$$
The decrease in $c(\alg)$ due to all of these swaps together is at least $c(\alg \setminus \sol)$ times some constant. In addition, since a swap between $a$ and $f$  increases $c'(\alg)$ by at most $c'(f)$, the total increase in $c'$ due to these swaps is at most $c'(\sol \setminus \alg)$ times some other constant. An averaging argument then gives the rate of exchange bound for the forward phase in the claim, as desired. The rate of exchange bound for the backward phase follows analogously.

This completes the algorithm and proof summary, although more detail is needed to formalize these arguments. Moreover, we also need to show that the algorithm runs in polynomial time. These details are given in Appendix~\ref{section:deferred-st}.


%This proof has three key parts: (a) We extend the charging analysis of \cite{GGKMSSV17} to show that being ``approximately locally optimal'' still gives some approximation guarantee. (b) We show that the contrapositive of this approximation guarantee combined with an averaging argument lets us relate our current difference approximation to the best ``rate of exchange'' of $c$ and $c'$ of any swap. (c) Finally, we use this to bound the decrease in $c(\alg)$ in a forward phase and increase in $c(\alg)$ in a backward phase, and thus show the net decrease is a non-negligible positive amount when \eqref{eq:maincond} holds.

% To prove (a): Suppose instead of considering all improving swaps, our local search only considered swaps between $S, f$ where $f$ has cost at most $1/\lambda$ times that of $S$, and we were fine with a solution for which a weighted fraction $1/\theta$ of the edges could not be swapped out in this manner (rather than all the edges as in a locally optimal solution). An extension of the analysis in \cite{GGKMSSV17} gives that a solution of this kind would still be a $14\lambda\theta$-approximation. 

% To prove (b), we observe the contrapositive of (a): While $\alg$ is not a $14\lambda\theta$-approximation, the weighted fraction of swaps we can make for which $c(S) > \lambda c(f)$ (i.e., for which the decrease in $c(\alg)$ is at least $(1-1/\lambda) \cdot c(S)$) is at least $1 - 1/\theta$. We leverage this fact to show that in the context of optimizing two costs at once, a swap exists that has a good ``rate of exchange'', i.e., decreases $c$ without increasing $c'$ too much. Namely, setting $\lambda, \theta = \sqrt{\Gamma}$, (a)'s contrapositive gives that while $\alg$ is not a $14\Gamma$-approximation, the total decrease in $c(\alg)$ across all (substantially improving) swaps with $\sol$ is at least some constant (depending on $\Gamma$) times $c(\alg \setminus \sol)$. We can use the fractional charging to show that the total increase in $c'(\alg)$ in swaps with $\sol$ is bounded by some constant times $c'(\sol \setminus \alg)$. So the ratio of decrease in $c$ to increase in $c'$ for the swap with the best ``rate of exchange'' can be lower bounded by some constant times $\frac{c(\alg \setminus \sol)}{c'(\sol \setminus \alg)}$ by an averaging argument. This argument is agnostic to the costs used, i.e. we can swap $c$ and $c'$ in the argument and it still holds. 

% To prove (c): (b) gives that in a forward phase, our rate of exchange (decrease in $c$ divided by increase in $c'$) for each swap is at least some constant times $\frac{c(\alg \setminus \sol)}{c'(\sol \setminus \alg)}$. Since (b) is agnostic to the cost functions used, it also gives that in a backward phase the rate of exchange (increase in $c$ divided by decrease in $c'$) for each swap is upper bounded by some constant times $\frac{c(\sol \setminus \alg)}{c'(\alg \setminus \sol)}$. If our lower threshold is sufficiently large, then $c'(\alg \setminus \sol)$ is much larger than $c'(\sol \setminus \alg)$, and the numerator is at most $\frac{1}{14\Gamma} c(\alg \setminus \sol)$ by assumption. This gives that the rate of exchange is upper bounded by $\frac{1}{14\Gamma} \frac{c(\alg \setminus \sol)}{c'(\sol \setminus \alg)}$ times some constant approaching 0 as $\Gamma$ approaches infinity, i.e. the lower bound for the rate of exchange in the forward phase times a constant we can make arbitrarily close to 0 by making $\Gamma$ large. In turn, this implies that if $\Gamma$ is sufficiently large, the swaps in the forward phase are making much more progress in improving $c$ than is undone by the swaps in the backward phase as desired. This completes the algorithm and proof summary, although more detail is needed to formalize these arguments. Moreover, we also need to show that the algorithm runs in polynomial time. These details are given in Appendix~\ref{section:deferred-st}.

% \debmalya{Parts (a), (b), (c) are not very clear, neither in the one-sentence summaries not in the more detailed paragraphs. Part of the problem is that there is some notation being introduced here that is new and therefore difficult to interpret for a reader. Can you rewrite this so that the exact flow of arguments is clear?}

We now formally define our separation oracle \textsc{RRST-Oracle} in Fig.~\ref{fig:storacle2} and prove that it is an approximate separation oracle in the lemma below:

\begin{figure}
\noindent
\fbox{\begin{minipage}{.98\textwidth}
\textsc{RRST-Oracle}($G(V, E)$, $\{[\ell_e, u_e]\}_{e \in E}$, $(\bx, r)$)\newline
\begin{algorithm}[H]
\KwData{Undirected graph $G(V, E)$, lower and upper bounds on edge lengths $\{[\ell_e, u_e]\}_{e \in E}$, solution ($\bx = \{x_e\}_{e \in E}, r$) to the LP in Fig.~\ref{fig:rrst}}
Check all constraints of the LP in Fig.~\ref{fig:rrst} except regret constraint set, \textbf{return} any violated constraint that is found\;
$G' \leftarrow $ copy of $G$ where $c_e = u_ex_e - \ell_ex_e + \ell_e$, $c_e' = \ell_e - \ell_e x_e$\;
$\alg \leftarrow $ output of algorithm from Lemma~\ref{lemma:differenceapprox2} on $G'$\;
\For{$\alg_i \in \alg$}{
\If{$\sum_{e \notin \alg_i} u_ex_e + \sum_{e \in \alg_i} \ell_ex_e - \sum_{e \in \alg_i} \ell_e > r$}{
\textbf{return} $\sum_{e \notin \alg_i} u_ex_e + \sum_{e \in \alg_i} \ell_ex_e - \sum_{e \in \alg_i} \ell_e \leq r$\;
}
}
\textbf{return} ``Feasible''\;
\end{algorithm}
\end{minipage}}
\caption{Separation Oracle for LP in Fig.~\ref{fig:rrst}}
\label{fig:storacle2}
\end{figure}

\begin{lemma}\label{lemma:steinersep2}
Fix any $\Gamma' > 1, \kappa > 0, 0 < \epsilon < 4/35$ and let $\Gamma$ be the constant given in Lemma~\ref{lemma:differenceapprox2}. Let $\alpha = (4\Gamma'+\kappa+2+\epsilon)4\Gamma+1$ and $\beta = 4\Gamma$. Then there exists an algorithm \textsc{RRST-Oracle} that given a solution $(\bx, r)$ to the LP in Fig.~\ref{fig:rrst} either:
\begin{itemize}
\item Outputs a separating hyperplane for the LP in Fig.~\ref{fig:rrst}, or
\item Outputs ``Feasible'', in which case $\bx$ is feasible for the (non-robust) Steiner tree LP and 
$$\forall \bd: \sum_{e \in E} d_e x_e \leq \alpha \cdot \opt (\bd) + \beta \cdot r.$$
\end{itemize}
\end{lemma}
\begin{proof}
It suffices to show that if there exists $\bd, \sol$ such that 
$$\sum_{e \in E} d_e x_e > \alpha \cdot \sol(\bd) + \beta \cdot r, \text { i.e., } \sum_{e \in E} d_ex_e - \alpha \cdot \sol(\bd) > \beta \cdot r$$ 
then \textsc{RRST-Oracle} outputs a violated inequality on line 6, i.e., the algorithm finds a Steiner tree $T'$ such that 
$$\sum_{e \notin T'} u_ex_e + \sum_{e \in T'} \ell_ex_e - \sum_{e \in T'} \ell_e > r.$$ 
Notice that in the inequality 
$$\sum_{e \in E} d_ex_e - \alpha \cdot \sol(\bd) > \beta \cdot r,$$ 
replacing $\bd$ with $\bd'$ where $d_e' = \ell_e$ when $e \in \sol$ and $d_e' = u_e$ when $e \notin \sol$ can only increase the left hand side. So replacing $\bd$ with $\bd'$ and rearranging terms, we have
$$\sum_{e \in \sol} \ell_ex_e + \sum_{e \notin \sol} u_ex_e > \alpha \sum_{e \in \sol} \ell_e + \beta \cdot r = \sum_{e \in \sol} \ell_e + \left[(\alpha-1) \sum_{e \in \sol} \ell_e + \beta \cdot r\right].$$
In particular, the regret of the fractional solution against $\sol$ is at least $(\alpha-1) \sum_{e \in \sol} \ell_e + \beta \cdot r$. 

Let $T'$ be the Steiner tree satisfying the conditions of Lemma~\ref{lemma:differenceapprox2} with $c_e = u_ex_e - \ell_ex_e + \ell_e$ and $c_e' = \ell_e - \ell_e x_e$. Let $E_0$ = $E \setminus (\sol \cup T')$, $E_S = \sol \setminus T'$, and $E_T = T' \setminus \sol$. Let $c(E')$ for $E' = E_0, E_S, E_T$ denote $\sum_{e \in E'} (u_ex_e - \ell_ex_e + \ell_e)$, i.e., the total weight of the edges $E'$ in $G'$. Now, note that the regret of the fractional solution against a solution using edges $E'$ is:

$$\sum_{e \notin E'} u_ex_e + \sum_{e \in E'} \ell_ex_e - \sum_{e \in E'} \ell_e = \sum_{e \notin E'} (u_ex_e - \ell_ex_e + \ell_e) - \sum_{e \in E}(\ell_e - \ell_ex_e) $$
$$= c(E \setminus E') - \sum_{e \in E}(\ell_e - \ell_ex_e).$$

Plugging in $E' = \sol$, we then get that:

$$c(E_0) + c(E_T) - \sum_{e \in E}(\ell_e - \ell_ex_e) > (\alpha - 1) \sum_{e \in \sol} \ell_e + \beta \cdot r.$$

Isolating $c(E_T)$ then gives:

$$c(E_T) > (\alpha - 1) \sum_{e \in \sol} \ell_e + \beta \cdot r - \sum_{e \in E_0} (u_ex_e  - \ell_e x_e + \ell_e) + \sum_{e \in E}(\ell_e - \ell_ex_e) $$
$$=(\alpha - 1) \sum_{e \in \sol} \ell_e + \beta \cdot r - \sum_{e \in E_0} u_ex_e + \sum_{e \notin E_0}(\ell_e - \ell_ex_e).$$

Since $\beta = 4\Gamma$, Lemma~\ref{lemma:differenceapprox2} along with an appropriate choice of $\epsilon$ gives that $c(E_{T}) \leq \beta c(E_{S})$, and thus:

$$c(E_S) > \frac{1}{\beta} \left[ (\alpha - 1) \sum_{e \in \sol} \ell_e + \beta \cdot r - \sum_{e \in E_0} u_ex_e + \sum_{e \notin E_0}(\ell_e - \ell_ex_e) \right].$$

Recall that our goal is to show that $c(E_0) + c(E_S) - \sum_{e \in E} (\ell_e - \ell_e x_e) > r$, i.e., that the regret of the fractional solution against $T'$ is at least $r$. Adding $c(E_0)- \sum_{e \in E} (\ell_e - \ell_e x_e)$ to both sides of the previous inequality, we can lower bound $c(E_0) + c(E_S) - \sum_{e \in E} (\ell_e - \ell_e x_e)$ as follows:

$$c(E_0) + c(E_S) - \sum_{e \in E} (\ell_e - \ell_e x_e) $$ 
$$> \frac{1}{\beta} \left[ (\alpha - 1) \sum_{e \in \sol} \ell_e + \beta \cdot r - \sum_{e \in E_0} u_ex_e + \sum_{e \notin E_0}(\ell_e - \ell_ex_e) \right]$$
$$+\sum_{e \in E_0} (u_e x_e  - \ell_e x_e + \ell_e) - \sum_{e \in E} (\ell_e - \ell_e x_e)$$
%$$= \frac{1}{\beta} \left[ (\alpha - 1) \sum_{e \in \sol} \ell_e + \beta \cdot r - \sum_{e \in E_0} u_ex_e + \sum_{e \notin E_0}(\ell_e - \ell_ex_e) \right]+\sum_{e \in E_0} u_e x_e - \sum_{e \notin E_0} (\ell_e - \ell_e x_e)$$
$$= r + \frac{\alpha-1}{\beta} \sum_{e \in \sol} \ell_e + \frac{1}{\beta}\sum_{e \notin E_0}(\ell_e - \ell_ex_e) +\frac{\beta - 1}{\beta} \sum_{e \in E_0} u_e x_e - \sum_{e \notin E_0} (\ell_e - \ell_e x_e)$$
$$\geq r + \frac{\alpha-1-\beta}{\beta} \sum_{e \in \sol} \ell_e + \frac{1}{\beta}\sum_{e \notin E_0}(\ell_e - \ell_ex_e) +\frac{\beta - 1}{\beta} \sum_{e \in E_0} u_e x_e - \sum_{e \in E_T} (\ell_e - \ell_e x_e) \geq r.$$
%$$\geq r + \frac{\alpha-1-\beta}{\beta} \sum_{e \in \sol} \ell_e - \sum_{e \in E_T} (\ell_e - \ell_e x_e)$$
%
Here, the last inequality holds because by our setting of $\alpha$, we have 
$$\frac{\alpha - 1 - \beta}{\beta} = 4\Gamma' + \kappa + 1 + \epsilon,$$ 
and thus Lemma~\ref{lemma:differenceapprox2} gives that $$\sum_{e \in E_T} (\ell_e - \ell_e x_e) \leq \frac{\alpha - 1 - \beta}{\beta}\sum_{e \in \sol} (\ell_e - \ell_e x_e) \leq \frac{\alpha - 1 - \beta}{\beta}\sum_{e \in \sol} \ell_e.$$
\end{proof}

By using Lemma~\ref{lemma:steinersep2} with the ellipsoid method and the fact that the LP optimum is at most $\mr$, we get an $(\alpha, \beta)$-robust fractional solution. Then, Theorem~\ref{thm:generalrounding} and known approximation/integrality gap results give us the following theorem, which with appropriate choice of constants gives Theorem~\ref{thm:steiner-main} (see Section~\ref{section:deferred-st} for details):

\begin{theorem}\label{thm:steiner}
Fix any $\Gamma' > 1, \kappa > 0, 0 < \epsilon < 4/35$ and let $\Gamma$ be the constant given in Lemma~\ref{lemma:differenceapprox2}. Let $\alpha = (4\Gamma'+\kappa+2+\epsilon)4\Gamma+1$ and $\beta = 4\Gamma$. Then there exists a polynomial-time $(2\alpha \ln 4 + \epsilon, 2 \beta \ln 4 + \ln 4+\epsilon)$-robust algorithm for the Steiner tree problem.
\end{theorem}
